SIFiD: Reassess Summary Factual Inconsistency Detection with LLM

Ensuring factual consistency between the summary and the original document is paramount in summarization tasks. Consequently, considerable effort has been dedicated to detecting inconsistencies. With the advent of Large Language Models (LLMs), recent studies have begun to leverage their advanced language understanding capabilities for inconsistency detection. However, early attempts have shown that LLMs underperform traditional models due to their limited ability to follow instructions and the absence of an effective detection methodology. In this study, we reassess summary inconsistency detection with LLMs, comparing the performances of GPT-3.5 and GPT-4. To advance research in LLM-based inconsistency detection, we propose SIFiD (Summary Inconsistency Detection with Filtered Document) that identify key sentences within documents by either employing natural language inference or measuring semantic similarity between summaries and documents.

==> table/ablation.tex <==
\begin{table}
\caption{Ablation study of Instruction Fusion. Models in the upper cell are 13B, while the models in the lower cell are 34B. ``-fused inst.'' represent model fine-tuned without corresponsding fused instructions.}
\small
\centering
\adjustbox{max width=\columnwidth}{
\begin{tabular}{l c c c c c}
\toprule
Method  & HumanEval & HumanEval$^+$ & MBPP & MBPP$^+$  \\
% \midrule
%     \textsc{CodeLlama-Python}-ECP*&13B 
%     &67.7&64.0&66.4&56.4\\
%     \textsc{CodeLlama}-ECP*&13B
%     &66.5&61.6&67.2&57.4\\
%     \textsc{CodeLlama}-EC*&13B
%     &65.2&61.0&68.4&56.1\\
% \midrule    
%     \textsc{CodeLlama-Python}-ECP*&34B 
%     &72.0&65.2&72.2&61.9\\
%     \textsc{CodeLlama}-ECP*&34B
%     &67.7&62.8&70.9&61.2\\  
%     \textsc{CodeLlama}-EC*&34B
%     &67.7&62.2&69.9&60.4\\
\midrule % code llama
    IF-CLP%&13B
    &\textbf{73.8} &\textbf{69.5} &\textbf{71.7} &\textbf{61.7}\\
    \ \ -fused inst.%&13B 
    &67.7&64.0&66.4&56.4\\
    % IF-CL-ECP%&13B 
    % &\textbf{75.6} &\textbf{68.9} &\textbf{67.9} &\textbf{58.6} \\
    % \ \ -fused inst.%&13B
    % &66.5&61.6&67.2&57.4\\
    IF-CL%&13B 
    &\textbf{74.4}&\textbf{68.3} &\textbf{69.7} &\textbf{59.4} \\  
    \ \ -fused inst.%&13B
    &65.2&61.0&68.4&56.1\\
\midrule
    IF-CLP%&34B
    &\textbf{75.6} &\textbf{69.5} &\textbf{73.7} &\textbf{62.7}\\
    \ \ -fused inst.%&34B 
    &72.0&65.2&72.2&61.9\\
    % IF-CL-ECP%&34B 
    % &\textbf{76.8} &\textbf{70.7} &\textbf{73.2} &\textbf{62.9}\\
    % \ \ -fused inst.%&34B
    % &{67.7} &{62.8} &{70.9} &{61.2}\\  
    IF-CL%&34B 
    &\textbf{78.7}&\textbf{71.3}&\textbf{71.4}&\textbf{60.7}\\
    \ \ -fused inst.%&34B
    &67.7&62.2&69.9&60.4\\
    % \midrule 
    % IF&Deepseek Coder&\CPI
    % &6.7B &xxxx&xxxx
    % &71.7&61.7\\
    
    % IF&Deepseek Coder&\CPI,\HPI
    % &6.7B &xxxx&xxxx
    % &73.7&63.2\\
    % \midrule
    \bottomrule 
\end{tabular}}

\label{tab-ablation}
\vspace{-5mm}
\end{table}

==> table/all.tex <==
\begin{table}[h]
\caption{Results of experiments using Magicoder dataset. All models are fine-tuned on \textsc{CodeLlama-Python}. `MC' represents the Magicoder dataset.}
\small
\centering
\adjustbox{max width=\columnwidth}{
\begin{tabular}{c c c c c c c c c}
\toprule
Method &Size & HumanEval($^+$) & MBPP($^+$)  \\\midrule
    Magicoder$\mathcal{S}$-CLP&7B
    &70.7(66.5)&68.4(56.6)\\    
    DeepSeek-Coder-instruct&33B
    &81.1(75.0)&78.7(66.7)\\
    WizardCoder-V1.1&33B
    &79.9(73.2)&78.9(66.9)\\\midrule
    IF-CLP-MC&7B
    &76.2(71.3)&{70.4}({57.9})\\
    IF-CLP-MC&13B
    &79.3(72.6)&{69.2}({57.4})\\
    IF-CLP-MC&34B
    &\textbf{82.3(75.6)}&\textbf{{72.4}({61.4})}\\
    \bottomrule 
\end{tabular}}
\label{tab-all}
\end{table}

==> table/multi.tex <==
\begin{table*}
\caption{Experiment results on the completion mode of MultiPL-E. Following the detailed experimental sitting of WizardCoder \cite{wizardcoder}, we employ \texttt{bigcode-evaluation-harness} \cite{bigcode} and report the other results from WiardCoder and Magicoder \cite{magicoder} paper.}
\small
\centering
\begin{tabular}{l c c c c c c c c}
\toprule
Method&Size & Java & JavaScript & C++ & PHP & Swift & Rust  \\
\midrule    
    \textsc{CodeLlama}&7B
    &29.3&31.7&27.0&25.1&25.6&25.5\\
    \textsc{CodeLlama-Python}&7B
    &29.1&35.7&30.2&29.0&27.1&27.0\\
    Magicoder$\mathcal{S}$-CLP&7B 
    &42.9&57.5&44.4&47.6&44.1&40.3\\
\midrule
    StarCoderBase&15B 
    &28.5&31.7&30.6&26.8&16.7&24.5\\
    StarCoder&15B 
    &30.2&30.8&31.6&26.1&22.7&21.8\\
    WizardCoder-SC&15B 
    &35.8&41.9&39.0&39.3&33.7&27.1\\
\midrule
    \textsc{CodeLlama}&34B
    &40.2&41.7&41.4&40.4&35.3&38.7\\
    \textsc{CodeLlama-Python}&34B 
    &39.5&44.7&39.1&39.8&34.3&39.7\\
    \textsc{CodeLlama-Instruct}&34B 
    &41.5&45.9&41.5&37.0&37.6&39.3\\
    WizardCoder-CLP&34B 
    &44.9&55.3&47.2&47.2&44.3&46.2\\


\midrule % code llama
    % \textsc{CodeLlama}-EC*&13B 
    % &39.8&55.3&47.2&44.7&41.8&23.6\\
    IF-CL-EC&13B
    &\textbf{45.3}&\textbf{64.6}&\textbf{54.6}&\textbf{53.4} &\textbf{50.0}&\textbf{54.5}\\
    \ \ -fused inst. &13B 
    &39.8&55.3&47.2&44.7&41.8&44.9\\
    \bottomrule 
\end{tabular}
\label{tab-multi}
% \vspace{-5mm}
\end{table*}

==> table/result_backup.tex <==
\begin{table*}
\caption{Results of experiments on Python benchmarks. The abbreviations 'CL' and 'CLP' denote the base models \textsc{CodeLlama} and \textsc{CodeLlama-Python}, respectively. 'EC' and 'ECP' represent the models fine-tuned with \texttt{evol-codealpaca-v1} and its Python-specific variant. Models and results marked with an asterisk '*' were reproduced by our team. The values in bracket indicate the performance improvement achieved by fine-tuning with instructions generated by IF, as compared to the use of \texttt{evol-codealpaca-v1} alone.}
\small
\centering
\begin{tabular}{l c c c c c c c c}
\toprule
Method &Size &Open-source& HumanEval & HumanEval+ & MBPP & MBPP+  \\\midrule
    GPT4-Turbo&- & -
    &85.4&81.7 &83.0&70.7\\
    GPT3.5-Turbo&-& -
    &72.6&65.9 &81.7&69.4\\
\midrule
    StarCoder&7B& weight\&data
    &24.4&20.7&33.1&28.8\\
    Mistral&7B& weight
    &28.7&23.2&50.1&40.9\\
    \textsc{CodeLlama-Python}&7B & weight
    &37.8&34.1&57.6&45.4\\
    WizardCoder-CLP&7B & weight
    &48.2&40.9&56.6&47.1\\
    Magicoder$\mathcal{S}$-CLP&7B& weight\&data
    &70.7&66.5&68.4&56.6\\
\midrule
    \textsc{CodeLlama-Python}&13B & weight
    &42.7&36.6&61.2&50.9\\
    WizardCoder-CLP&13B & weight
    &64.0&- \\
    StarCoder&15B & weight\&data
    &34.1&29.3&55.1&46.1 \\   
    CodeT5+&16B & weight\&data
    &31.7&26.2&54.6&44.4 \\
    CodeGen-Mono&16B & weight\&data
    &32.9&27.4&52.6&43.6 \\
    \textsc{CodeLlama-Python}-ECP*&13B &-
    &67.7&64.0&66.4&56.4\\
    \textsc{CodeLlama}-ECP*&13B &-
    &66.5&61.6&67.2&57.4\\
    \textsc{CodeLlama}-EC*&13B&-
    &65.2&61.0&68.4&56.1\\
\midrule    
    \textsc{CodeLlama-Python}&34B & weight
    &51.8&42.7&67.2&52.9\\   
    WizardCoder-CLP&34B & weight
    &73.2&64.6 &73.2&59.9\\
    \textsc{CodeLlama-Python}-ECP*&34B &-
    &72.0&65.2&72.2&61.9\\
    \textsc{CodeLlama}-ECP*&34B &-
    &67.7&62.8&70.9&61.2\\  
    \textsc{CodeLlama}-EC*&34B&-
    &67.7&62.2&69.9&60.4\\
\midrule % code llama
    IF-CLP-ECP&13B& weight\&data
    &73.8 (+6.1)&\textbf{69.5} (+5.5)&\textbf{71.7} (+5.3)&\textbf{61.7} (+5.3)\\
    IF-CL-ECP&13B & weight\&data
    &\textbf{75.6} (+9.1)&68.9 (+7.3) &67.9 (+0.7)&58.6 (+1.2)\\
    IF-CL-EC&13B & weight\&data
    &75.0 (+9.8)&68.9 (+7.9)&70.2 (+1.8)&59.4 (+3.3)\\  
\midrule
    IF-CLP-ECP&34B& weight\&data
    &75.6 (+3.6)&69.5 (+4.3)&\textbf{73.7} (+1.5)&62.7 (+0.8)\\
    IF-CL-ECP&34B & weight\&data
    &\textbf{76.8} (+9.1)&\textbf{70.7} (+7.9)&73.2 (+2.3)&62.9 (+1.7)\\
    IF-CL-EC&34B & weight\&data
    &75.0 (+7.3)&\text{70.1} (+7.9)&\textbf{73.7} (+3.8)&\textbf{63.9} (+3.5)\\
    % \midrule 
    % IF&Deepseek Coder&\CPI
    % &6.7B &xxxx&xxxx
    % &71.7&61.7\\
    
    % IF&Deepseek Coder&\CPI,\HPI
    % &6.7B &xxxx&xxxx
    % &73.7&63.2\\
    % \midrule
    \bottomrule 
\end{tabular}

\label{tab-python}
\vspace{-5mm}
\end{table*}

==> table/results.tex <==
\begin{table*}
\caption{Results of experiments on Python benchmarks. The abbreviations `CL' and `CLP' denote the base models \textsc{CodeLlama} and \textsc{CodeLlama-Python}, respectively. For IF method, we fine-tune \textsc{CodeLlama} with full \texttt{evol-codealpaca-v1} dataset and \textsc{CodeLlama-Python} with only Python instruction in \texttt{evol-codealpaca-v1}. }%The values in bracket indicate the performance improvement achieved by fine-tuning with instructions generated by IF, as compared to the use of \texttt{evol-codealpaca-v1} alone.}
\small
\centering
\begin{tabular}{l c c c c c c c c}
\toprule
Method &CoGenSum &XsumFaith& Polytope & FactCC & SummEval & FRANK&Avg.  \\\midrule
    GPT4-Turbo&- & -
    &85.4&81.7 &83.0&70.7\\
    GPT3.5-Turbo&-& -
    &72.6&65.9 &81.7&69.4\\
\midrule
    StarCoder&7B& weight\&data
    &24.4&20.7&33.1&28.8\\
    Mistral&7B& weight
    &28.7&23.2&50.1&40.9\\
    \textsc{CodeLlama-Python}&7B & weight
    &37.8&34.1&57.6&45.4\\
    WizardCoder-CLP&7B & weight
    &48.2&40.9&56.6&47.1\\
    Magicoder$\mathcal{S}$-CLP&7B& weight\&data
    &70.7&66.5&68.4&56.6\\
\midrule
    \textsc{CodeLlama-Python}&13B & weight
    &42.7&36.6&61.2&50.9\\
    % WizardCoder-CLP&13B & weight
    % &64.0&- \\
    StarCoder&15B & weight\&data
    &34.1&29.3&55.1&46.1 \\   
    CodeT5+&16B & weight\&data
    &31.7&26.2&54.6&44.4 \\
    CodeGen-Mono&16B & weight\&data
    &32.9&27.4&52.6&43.6 \\
    % \textsc{CodeLlama-Python}-ECP*&13B &-
    % &67.7&64.0&66.4&56.4\\
    % \textsc{CodeLlama}-ECP*&13B &-
    % &66.5&61.6&67.2&57.4\\
    % \textsc{CodeLlama}-EC*&13B&-
    % &65.2&61.0&68.4&56.1\\
\midrule    
    \textsc{CodeLlama-Python}&34B & weight
    &51.8&42.7&67.2&52.9\\   
    WizardCoder-CLP&34B & weight
    &73.2&64.6 &73.2&59.9\\
    % \textsc{CodeLlama-Python}-ECP*&34B &-
    % &72.0&65.2&72.2&61.9\\
    % \textsc{CodeLlama}-ECP*&34B &-
    % &67.7&62.8&70.9&61.2\\  
    % \textsc{CodeLlama}-EC*&34B&-
    % &67.7&62.2&69.9&60.4\\
\midrule % code llama
    IF-CLP&13B& weight
    &73.8 &\textbf{69.5}&\textbf{71.7}&\textbf{61.7}\\
    % IF-CL-ECP&13B & weight\&data
    % &\textbf{75.6}&68.9&67.9&58.6\\
    IF-CL&13B & weight
    &\textbf{74.4}&68.3&69.7&59.4\\  
\midrule
    IF-CLP&34B& weight
    &75.6&69.5&\textbf{73.7}&62.7\\
    % IF-CL-ECP&34B & weight\&data
    % &{76.8}&{70.7}&73.2&\textbf{62.9}\\
    IF-CL&34B & weight    &\textbf{78.7}&\textbf{71.3}&71.4&{60.7}\\
    % \midrule 
    % IF&Deepseek Coder&\CPI
    % &6.7B &xxxx&xxxx
    % &71.7&61.7\\
    
    % IF&Deepseek Coder&\CPI,\HPI
    % &6.7B &xxxx&xxxx
    % &73.7&63.2\\
    % \midrule
    \bottomrule 
\end{tabular}

\label{tab-python}
\vspace{-5mm}
\end{table*}
